Pythia: Grammar-Based Fuzzing of REST APIs with Coverage-guided Feedback and Learning-based Mutations

This paper introduces Pythia, the first fuzzer that augments grammar-based fuzzing with coverage-guided feedback and a learning-based mutation strategy for stateful REST API fuzzing. Pythia uses a statistical model to learn common usage patterns of a target REST API from structurally valid seed inputs. It then generates learning-based mutations by injecting a small amount of noise deviating from common usage patterns while still maintaining syntactic validity. Pythia's mutation strategy helps generate grammatically valid test cases and coverage-guided feedback helps prioritize the test cases that are more likely to find bugs. We present experimental evaluation on three production-scale, open-source cloud services showing that Pythia outperforms prior approaches both in code coverage and new bugs found. Using Pythia, we found 29 new bugs which we are in the process of reporting to the respective service owners.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf .out .aux

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = paper

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		$(name).out \
		psfig.aux \
		*.bbl \
		*.pdfsync

#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf:
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> sections/03-05-coverage-monitor.tex <==
\subsubsection{Coverage Monitor}
\label{sec:coverage-monitor}

In this step, we monitor whether an executing test case increases code coverage, i.e., reaches new basic blocks, in general. To do that, first, we instrument target services before fuzzing and then during fuzzing dynamically collect coverage information. For instrumentation, we statically analyze the source code of the target and extract basic block locations. Next, during fuzzing, we configure Ruby's {\tt Class:TracePoint} hooks to trace which lines of code are executed by each test case, and then identify the respective basic blocks.  This step is similar to AFL's instrumentation on native C binaries~\cite{afl}.
However, since we apply this methodology on interpreted code, we may
potentially miss some basic blocks that are defined within complex if-else list comprehension structures~\vlis{We can move this statement to threats to validity}. Using basic block coverage information,
we further distill the test cases that reach new basic blocks, and these distilled test cases are used for incrementally training the model, as explained in~\S\ref{sec:training-engine}.

% We instrument target services and dynamically collect coverage
% information during fuzzing. To achieve this, before fuzzing, we statically
% analyze the source code of the target and
% extract basic block locations (i.e., codes sequence
% with no branches in and out except to the entry and at the end respectively).
% Afterwards, during fuzzing, we configure Ruby's {\tt Class:TracePoint} hooks to
% trace which lines of code (and from what files) are executed by each test case,
% and then match the executed lines of code with their respective basic blocks.
% This step is similar to AFL's instrumentation on native C binaries~\cite{afl}.
% However, since we apply this methodolody on interpreted code, we may
% potentially miss a subset of basic block that are defined within complex if-else
% list comprehension structures. Using basic block coverage information,
% we distill test cases to a smaller set of test cases that active
% new basic blocks, and the distilled new test cases are being used by the
% {\it training engine} to learn new models and update old ones, as explained
% in~\S\ref{sec:training-engine}.


==> sections/04-evaluation-back.tex <==
\begin{figure*}[t]
    \begin{minipage}{\textwidth}
    \centering
    \subfigure{
        \includegraphics[width=0.31\textwidth]{figures/commits_merged.pdf}
    }
    \subfigure{
        \includegraphics[width=0.31\textwidth]{figures/branches_merged.pdf}
    }
    \subfigure{
        \includegraphics[width=0.31\textwidth]{figures/issues_notes_merged.pdf}
    }

    \medskip
    \subfigure{
        \includegraphics[width=0.31\textwidth]{figures/repositories_repository_file_merged.pdf}
    }
    \subfigure{
        \includegraphics[width=0.31\textwidth]{figures/projects_and_projectsm_merged.pdf}
    }
    \subfigure{
        \includegraphics[width=0.31\textwidth]{figures/groups_members_merged.pdf}
    }
    \vspace{-5pt}
    \caption{
        {\bf Comparison of \pythia mutations strategies.}
        \underline{Seed collection:} Run \restler on each API in order
        to generate seed test case corpuses. The seed collection time is
        set to $24$h for all APIs expect for ``issues" in which the respective
        time was extended to $32$h.
        Within $24$h \restler reached a plateau in all APIs except for issues,
        where the respective time had to be extended to $32$h due to a later
        plateau.
        \underline{Fuzzing:} Use each corpus to perform three individual
        $24$h fuzzing sessions per API.
        %: one for each mutation strategy,
        %including random
        %byte-level, random tree-level, and guided tree-level mutations.
        Moreover, let \restler run for $24$h additional hours ($48$h in total).
        \underline{Comparison:} Show the number of new lines executed after the
        initial seed collection. Note that \restler is run for $48$h in
        total but no new lines are discovered, for no API, in the later $24$h
        shown in the graphs. Whereas, \pythia fuzzers are run for $24$h,
        mutating the seed corpuses generated by the first $24$h of RESTler
        traffic, and discover new lines that have not been covered before.
    }
    \label{fig:all-distillation-off}
    \end{minipage}\\[1em]
\end{figure*}


\section{Results}
\label{sec:results}


\input{sections/05-01-mutations}
\input{sections/05-02-seeds-volume}
\input{sections/05-03-optimizations}
\input{sections/05-04-restler-modes}


==> sections/04-experiment-design-back.tex <==
\section{Experimental Setup}
% We describe the experimental set up of our evaluation including
% the set up of the target service deployments, the fuzzing set up,
% and the configuration and hyper-parameters of
% the ML models used.

%\heading{Target service deployments.}
\subsection{Study Subject}
\label{sec:subj}

~\Cref{tab:target-apis} summarizes the APIs tested by \pythia. We tested 6 APIs of \gitlab, 2 APIs of Mastodon, and 1 API from Spree\vlis{check if this is correct}.

First, we test
\gitlab enterprise edition stable version 11-11 through its REST APIs related
to common version control operations. \gitlab is an open-source web service
for self-hosted Git, its
back-end is written in over 376K lines of ruby code using ruby-on-rails, and
its functionality is exposed through a REST API. GitLab [13] is used by more
than 100,000 organizations, has millions of users, and has currently a 2/3
market share of the self-hosted Git market [20]. We apply the following
configuration settings: we use Nginx HTTP web server and
configure rails with 20 Unicorn workers limited to up to 4GB of physical memory;
we use
postgreSQL for persistent storage configured with a pool of 20 workers;
we use GitLab’s default configuration for sidekiq queues and redis workers as
well as the Nginx HTTP server.
According to GitLab’s deployment recommendations, such configuration
should scale up to 4,000 concurrent users [15].
Second, we test Mastodon~\cite{mastodon}, an open-source, self-hosted social
networking service. \vlis{talk about Spree}
%

\Cref{tab:target-apis} shows the characteristics of the target service APIs
under tests. All target APIs are related to common operation the users of the
corresponding services may do. In principal, the total number of requests in
each API family along with the average number of available primitive value
combinations for each request indicate the size of the state space that needs
to be tested. Furthermore, the existence of path, body dependencies, or both,
among request types capture another qualitative property indicative of how
difficult it is to generate sequences of request combinations.



\begin{table}[t]
{
    \small
    %\def\arraystretch{1.2}
    \begin{center}
        %\begin{tabular}{p{1.2cm} p{2.5cm} p{1.22cm} p{2cm}}
        \begin{tabular}{llrr}
            \toprule
            %{\bf Target Service}            &   {\bf API Family}        &{\bf Total Requests}
            %&{\bf Request Dependencies}\\
            {\bf Target }   &   {\bf API }    & {\bf Total }     & {\bf Request }\\
            {\bf  Service}  &   {\bf  Family} & {\bf  Requests}  & {\bf  Dependencies}\\
            \midrule
            \multirow{1}{*}{\bf GitLab}
                &   Commits                 & 15~(*11)                  & Path, Body\\
                &   Brances                 & 8~~(*2)                   & Path\\
                &   Issues \& Notes         & 25~(*20)                  & Path\\
                &   User Groups             & 53~(*2)                   & Path\\
                &   Projects \& Files       & 54~(*5)                   & Path\\
                &   Repos \& Files          & 12~(*22)                  & Path\\
			\midrule
            \multirow{1}{*}{\bf Mastodon}
                &   Accounts \& Lists       & 26~(*5)                    & Path, Body\\
                &   Statuses                & 18~(*26)                   & Path\\
			\midrule
            \multirow{1}{*}{\bf Spree}
                &   Products \& Carts       & 19                         & Path\\
            \bottomrule
        \end{tabular}
        \caption{{\bf Target service APIs.}
            For each target service, the number of
            distinct request types in each API family and (*) the average number
            of primitive value combinations that are available for each request
            type is shows as well as whether each API family has requests with
            path or body dependencies, or both.
        }
        \label{tab:target-apis}
    \end{center}
    \vspace{-23pt}
}
\end{table}

\subsection{Coverage monitoring \& Initial seed generation}\vlis{We need a better name, may be Monitoring Framework?}

All target services tested are monitored by \pythia's {\em coverage monitor}.
\vlis{Perhaps describe the coverage montitor here a bit.}
In GitLab, the {\em coverage monitor} traces all modules defined in
{\tt /lib} and {\tt /app} folders. In order to perform seed distillation,
we statically analyze the source code of the particular modules and extract
11,413 basic for \gitlab, 6,000 basic blocks for \mastodon, and \vlis{XXX} basic blocks for Spree.

\pythia starts fuzzing using an initial corpus
of seeds generated by \restler, an existing, stateful REST API fuzzer\vlis{cite}. To produce
these initial seeds, we run \restler for a custom amount of time on each
individual API family of each target service using its
default fuzzing mode (\ie Breadth First Search), its default fuzzing dictionary
(\ie two values for each primitive type), and by turning off its Garbage
Collector (GC) to obtain more deterministic results.

% \heading{Seq2seq models.}
% We use an off-the-shelf seq2seq RNN
% with input embedding, implemented in tensorflow~\cite{tensorflow}.
% The model has one layer of  $256$ Gated Recurrent Unit (GRU) cell in the encoder
% as well as in the decoder. Dynamic input unrolling is performed using
% {\tt tf.nn.dynamic} RNN APIs and the encoder is initialized with a zero state.
% We train the model by minimizing the weighted cross-entropy loss for sequences
% of logits using the Adam optimizer~\cite{adam}. We use batches of $32$
% sequences, iterate for $2000$ training steps with a learning rate of $0.001$,
% and an initial embedding layer of size $100$. The vocabulary of the model
% depends on the number of production rules in the fuzzing grammar of each API
% family and ranges in couple of hundred of production rules. Similarly, the
% length of each sequence depends on the specific API and ranges from
% 500 to 780 rules.
% %
% % [VA]: specify the APIs.
% %
% Training such a model configuration
% in a CPU-only machine takes no more than two hours.
% All the experiments discussed in our evaluations were run on Ubuntu 18.04
% Google Cloud VMs~\cite{google-cloud} with 8 logical CPU cores
% and 52GB of physical memory.
% %, without any Graphics Processing Unit (GPU) acceleration.
% Each fuzzing client is used to test a target
% service deployment running on the same machine.

\subsection{Evaluating \pythia}

\subsection*{Baselines.} To evaluate \pythia's mutation strategy w.r.t.~three  baselines: (i) \restler, (ii) random byte-level mutation strategy, and
(iii) random tree-level mutation strategy.


\noindent
(i) \heading{Restler.} \vlis{refer and summarize}

\noindent
(ii) \heading{Random byte-level mutations.}
This is the simplest form of mutations. % performed by \pythia.
As suggested by their name, byte-level mutations are random alternations on the bytes of each seed test case.
%Recall from the example test case shown in the left-hand side of~\F\ref{fig:abstraction-engine-example} that, before abstraction, each test case is practically a sequence of bytes.
In order to produce byte-level mutations, the {\it mutation engine} selects a random target position
within the seed sequence and a random byte value (in the range $0-255$),
and updates the target position to the random byte value.
Naturally, this type of mutations are not always syntactically or semantically
valid (defined in~\S\ref{sec:motivation}).
%and we will see later on (\S\ref{sec:evaluation} and~\S\ref{sec:case-studies}) how this strategy performs in terms of code coverage and new bugs found.

\noindent
(iii) \heading{Random tree-level mutations.}
The second type of mutations is random, tree-level mutations performed on the
leaves of the tree representations of each seed test case.
Given a time budget, Algorithm~\ref{alg:random-tree-mutations}
continuously iterates over the corpus of available seed test cases $\mathcal{S}$ by using
function $get\_next$. Each seed test case is mapped to its respective tree
representation deonoted $\mathcal{X}$ (using function $\mathcal{AST}$) and a
random leaf position as well as a random, new rule with terminal symbol
from $\mathcal{G}$ are selected. The current seed is then updated with a new
leaf mutation resulting to a new test case. At the end of each iteration,
the updated seed (new test case) is executed to
the target service by function {\em EXECUTE}, implemented in the
{\it execution engine}.\vlis{update this step, it is refering to some obsolete algo}

The mutations are exclusively performed on the tree leafs, and not in internal nodes,
in order to maintain semantic validity of each test case.
However, since the target leafs and the new rules (mutations) are selected
at random for each test case, the target state space for mutations
on realistic tests cases is quite large.
For example, the test case show in~\F\ref{fig:testcase} is represented to a tree
that consisting of 73 leaf nodes and the RG used to produce it has 66 rules with
terminal rules. This, defines a state space of almost 5,000 feasible mutations
only for one seed --- let alone the total size of the state space defined by the
complete corpus of seeds. Next, we introduce a learning-based mutation
strategy which considers the intrinsic characteristics of each test case and
significantly prunes the size of the search space.



\subsubsection{Evaluation}
\label{sec:evaluation}

We present experimental results obtained with \pythia that answer the following questions:
\begin{enumerate}
    \item[\underline{{\bf Q1:}}] How do the three mutation strategies
        implemented in \pythia (random byte-level mutations, random tree-level
        mutations, and guided tree-level mutations) comparatively increase
        code coverage over time?
        (Section~\ref{sec:evaluation:mutations})
    \item[\underline{{\bf Q2:}}] How does the volume of initial seeds impacts
        the code coverage achieved by \pythia?
        (Section~\ref{sec:evaluation:seeds-volume})
    \item[\underline{{\bf Q3:}}] What is the benefit offered by seed
        distillation?
        (Section~\ref{sec:evaluation:optimizations:distillation})
    \item[\underline{{\bf Q4:}}] What is the benefit offered by model
        retraining?
        (Section~\ref{sec:evaluation:optimizations:retraining})\vlis{change}
%    \item[\underline{{\bf Q5:}}] How does pythia compare with various \restler
%        fuzzing modes?
%        (Section~\ref{sec:evaluation:restler-modes})

\end{enumerate}

